Measurement of the inclusive jet cross-sections in proton--proton collisions at $\sqrt{s}= $8 TeV with the ATLAS detector

Inclusive jet production cross-sections are measured in proton--proton collisions at a centre-of-mass energy of $\sqrt{s}=$8 TeV recorded by the ATLAS experiment at the Large Hadron Collider at CERN. The total integrated luminosity of the analysed data set amounts to $20.2$ fb$^{-1}$. Double-differential cross-sections are measured for jets defined by the anti-$k_{t}$ jet clustering algorithm with radius parameters of $R=0.4$ and $R=0.6$ and are presented as a function of the jet transverse momentum, in the range between 70 GeV and 2.5 TeV and in six bins of the absolute jet rapidity, between 0 and 3.0. The measured cross-sections are compared to predictions of quantum chromodynamics, calculated at next-to-leading order in perturbation theory, and corrected for non-perturbative and electroweak effects. The level of agreement with predictions, using a selection of different parton distribution functions for the proton, is quantified. Tensions between the data and the theory predictions are observed.

==> atlas_inclusive_jet2012_antiktr04_pereventscale_eta1eta2eta3eta4eta5eta6_ptCut1_SplitSyst_ExpAndTh.tex <==
% pTcut1
% R=0.4 and R=0.6  $P_{T,jet,max}$ \\
% data-file name: Data/jet/atlas/incljets2012//atlas_2012_jet_antiktr06_incljetpt_eta1_highmu.txt
% grid-file name: Grids/jet/atlas/incljets2012/nlojet/pereventscale/atlas_2012_jet_antiktr06_incljetpt_eta1.txt
% PDF: CT14
% correction k^{A14}_{NP}
 Splitting options for $R=0.4$  & CT14 & NNPDF3.0 \\
 \hline  
        JES Flavour Response Opt 7  \\
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES MJB Fragmentation Opt 17   \\ 
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES Pile-up Rho topology Opt 18   \\  
% 18 \hspace{0cm}                
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 2 ) ^2 } \cdot $  uncertainty   \\
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 2, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Scale variations Opt 17 \\  
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Alternative scale choice Opt 7  \\ 
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Non-perturbative corrections Opt 7
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty
                                          & 268/159     & 257/159     \\
 \hline
 \hline
        JES Flavour Response Opt 7  \\
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES MJB Fragmentation Opt 17   \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES Pile-up Rho topology Opt 18   \\
% 18 \hspace{0cm}                
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 2 ) ^2 } \cdot $  uncertainty   \\
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 2, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Scale variations Opt 20 \\
%%       $ f_1(\pt,y) = C(\pt,y) \cdot  9.62 \cdot 10^{-2} / log \left( M(y) / \pt \right) \cdot $ uncertainty \\
%%       $ f_2(\pt,y) = C(\pt,y) \cdot  2.89 \cdot 10^{-2} \cdot y^2 / log \left( M(y) / \pt \right) \cdot $ uncertainty \\
%%       $ f_3(\pt,y) = C(\pt,y) \cdot  8.42 \cdot 10^{-2} \cdot $ uncertainty \\
%%       $ f_4(\pt,y) = C(\pt,y) \cdot  0.842 \cdot 10^{-2} \cdot y^2 \cdot $ uncertainty \\
%%       $ f_5(\pt,y) = C(\pt,y) \cdot  1.68 \cdot 10^{-2} \cdot log \left( 15 \pt / M(y) \right) \cdot $ uncertainty \\
%%       $ f_6(\pt,y) = C(\pt,y) \cdot  0.336 \cdot 10^{-2} \cdot y^2 log \left( 15 \pt / M(y) \right) \cdot $ uncertainty \\
% $( 9.62 \cdot 10^{-2}, 2.89 \cdot 10^{-2}, 8.42 \cdot 10^{-2}, 0.842 \cdot 10^{-2}, 1.68 \cdot 10^{-2}, 0.336 \cdot 10^{-2} )$ for option 20
 \cline{1-1}
        Alternative scale choice Opt 17 \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Non-perturbative corrections Opt 7  
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty
                                                   & 261/159     & 260/159     \\


==> atlas_inclusive_jet2012_antiktr04r06_PereventPerjetScales_eta1eta2eta3eta4eta5eta6_highmu.tex <==
% several pT cuts
% R=0.4 and R=0.6  $P_{T,jet,max}$ $P_{T,jet}$ \\
% data-file name: Data/jet/atlas/incljets2012//atlas_2012_jet_antiktr06_incljetpt_eta1_highmu.txt
% grid-file name: Grids/jet/atlas/incljets2012/nlojet/pereventscale/atlas_2012_jet_antiktr06_incljetpt_eta1.txt
% PDF: CT14
% correction k^{A14}_{NP}
 $\chi^2$/ndf  & \pTjetmax &  & \pTjet & \\
 {}            & $R=0.4$ & $R=0.6$ & $R=0.4$ & $R=0.6$ \\
 \hline  
{} $\pt > 70$~\GeV \hspace{0cm} \\
     CT14
                & 349/171  
                & 398/171  
                & 340/171  
                & 392/171   \\
 \hline  
HERAPDF2.0
                & 415/171  
                & 424/171  
                & 405/171  
                & 418/171   \\
 \hline  
  NNPDF3.0
                & 351/171  
                & 393/171  
                & 350/171  
                & 393/171   \\
 \hline  
 MMHT2014
                & 356/171  
                & 400/171  
                & 354/171  
                & 399/171   \\
 \hline  
\ptcut{ptcut1} \hspace{0cm} \\
     CT14
                & 321/159  
                & 360/159  
                & 313/159  
                & 356/159   \\
 \hline  
HERAPDF2.0
                & 385/159  
                & 374/159  
                & 377/159  
                & 370/159   \\
 \hline  
  NNPDF3.0
                & 333/159  
                & 356/159  
                & 331/159  
                & 356/159   \\
 \hline  
 MMHT2014
                & 335/159  
                & 364/159  
                & 333/159  
                & 362/159   \\
 \hline  
\ptcut{ptcut2} \hspace{0cm} \\
     CT14
                & 272/134  
                & 306/134  
                & 262/134  
                & 301/134   \\
 \hline  
HERAPDF2.0
                & 350/134  
                & 331/134  
                & 340/134  
                & 326/134   \\
 \hline  
  NNPDF3.0
                & 289/134  
                & 300/134  
                & 285/134  
                & 299/134   \\
 \hline  
 MMHT2014
                & 292/134  
                & 311/134  
                & 284/134  
                & 308/134   \\
 \hline  
\ptcut{ptcut3} \hspace{0cm} \\
     CT14
                & 128/72  
                & 149/72  
                & 118/72  
                & 145/72   \\
 \hline  
HERAPDF2.0
                & 148/72  
                & 175/72  
                & 141/72  
                & 170/72   \\
 \hline  
  NNPDF3.0
                & 119/72  
                & 141/72  
                & 115/72  
                & 139/72   \\
 \hline  
 MMHT2014
                & 132/72  
                & 143/72  
                & 122/72  
                & 140/72   \\
 \hline  



==> atlas_inclusive_jet2012_antiktr06_pereventscale_eta1eta2eta3eta4eta5eta6_ptCut1_SplitSyst_ExpAndTh.tex <==
% pTcut1
% R=0.4 and R=0.6  $P_{T,jet,max}$ \\
% data-file name: Data/jet/atlas/incljets2012//atlas_2012_jet_antiktr06_incljetpt_eta1_highmu.txt
% grid-file name: Grids/jet/atlas/incljets2012/nlojet/pereventscale/atlas_2012_jet_antiktr06_incljetpt_eta1.txt
% PDF: CT14
% correction k^{A14}_{NP}
 Splitting options for $R=0.6$  & CT14 & NNPDF3.0 \\
 \hline  
        JES Flavour Response Opt 14  \\
% 14 \hspace{0cm}
%%        $ L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES MJB Fragmentation Opt 17  \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES Pile-up Rho topology Opt 16   \\
% 16 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1.5 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1.5, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Scale variations Opt 17 \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Alternative scale choice Opt 16 \\
% 16 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1.5 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1.5, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Non-perturbative corrections Opt 18
% 18 \hspace{0cm}                
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 2 ) ^2 } \cdot $  uncertainty   \\
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 2, 3 ) \cdot $  uncertainty
               & 266/159     & 258/159     \\
 \hline
 \hline
        JES Flavour Response Opt 7   \\
% 7 \hspace{0cm}
%%        $ L( |y|, 0, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES MJB Fragmentation Opt 17  \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        JES Pile-up Rho topology Opt 16   \\
% 16 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1.5 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1.5, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Scale variations Opt 17 \\
% 17 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Alternative scale choice Opt 16 \\
% 16 \hspace{0cm}
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 1.5 ) ^2 } \cdot $  uncertainty   \\
%%        $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 1.5, 3 ) \cdot $  uncertainty   \\
 \cline{1-1}
        Non-perturbative corrections Opt 18
% 18 \hspace{0cm}                
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  \sqrt{ 1 - L( |y|, 0, 2 ) ^2 } \cdot $  uncertainty   \\
%%         $ \sqrt{ 1 - L( {\rm ln}(\pt{}[\TeV]), {\rm ln}(0.1), {\rm ln}(2.5) ) ^2 } \cdot  L( |y|, 2, 3 ) \cdot $  uncertainty
               & 264/159     & 256/159     \\


==> systematicstable.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|}
\hline
\hline
 Name                  &    $N$  &  Description \\
\hline
%
\hline
Jet energy scale (JES) & & \\
\hline
    \zjet{} balance   &  & \\
%
JES  Zjet  MuScale    &  1  & Baseline uncertainty in muon energy scale \\
%
JES  Zjet  MuSmearID  &  1  & Uncertainty in muon inner detector (ID) momentum smearing \\
%
JES  Zjet  MuSmearMS  &  1  & Uncertainty in muon system (MS) momentum smearing \\
%
JES  Zjet  Veto       &  1  & Variation in sub-leading jet veto (radiation suppression) \\
%
JES  Zjet  dPhi       &  1  & Extrapolation in $\Delta \Phi$ \\
%
JES  Zjet  MC         &  1  & Difference between MC event generators \\ 
%
JES  Zjet  OOC        &  1  & Contribution of particles outside the jet cone \\
%
JES  Zjet  JVF        &  1  & JVF choice: Jet selection to suppress pile-up jets \\
%
JES  Zjet  Stati      &  11  & Statistical uncertainty eigenvector $i=1,11$  \\
%
\hline
 \gjet{} balance  &  & \\
%
JES  Gjet  Veto       &  1  & Variation in sub-leading jet veto (radiation suppression) \\
%
JES  Gjet  dPhi       &  1  & Extrapolation in $\Delta \Phi$ \\
%
JES  Gjet  Generator  &  1  & Difference between MC event generator \\
%
JES  Gjet  OOC        &  1  & Contribution of particles outside the jet cone \\
%
JES  Gjet  Purity     &  1  & Photon purity of \gjet{} sample (background from multi-jet events) \\  
%
JES  Gjet  Stati      & 13  & Statistical uncertainty eigenvector $i=1,13$  \\
%
\hline
Multi-jet balance &  & \\
%
JES  MJB  Alpha         & 1 & Angle between leading jet and recoil system \\
%
JES  MJB  Beta          & 1 & Angle between leading jet and closest sub-leading jet \\
%
JES  MJB  Fragmentation & 1 & Difference between MC event generators (fragmentation) \\
%
JES  MJB  Asym          & 1 & Symmetry selection between leading and sub-leading jet \\
%
JES  MJB  Threshold     & 1 & Jet \pt~threshold \\
%
JES  MJB  Stati         & 10 & Statistical uncertainty eigenvector $i=1,13$ \\
%
\hline
Common sources in \zjet{} and \gjet{} balance   &  & \\
%
JES  LArEsmear             & 1  & Uncertainty in electron and photon energy smearing      \\
%
JES  LArESmaterial         & 1  & Material uncertainty in photon and energy energy scale  \\
%
JES  LArESpresampler       & 1  & Pre-sampler calibration uncertainty in photon and electron energy scale \\
%
JES  LArESZee              & 1  & Baseline uncertainty in electron and photon energy scale \\ 
%
\hline
  Di-jet $\eta$-intercalibration & & \\
%
JES  EtaIntercalibration  Modelling &  1 & MC generator modelling uncertainty in $\eta$-intercalibration \\
%
JES  EtaStati                       &  240/250 & Statistical uncertainty $i=0-239/249$ (one per \insitu{} analysis bin) \\
%
\hline
  High-\pt{} jets  & & \\
%
JES  SingleParticle  HighPt         &  1 & High-\pt{} calibration from single particle response \\
JES  Punch  through                 &  1 & High-\pt{} punch-through uncertainty  \\
%
\hline
 Pile-up substraction   & & \\
%
JES  Pile-up  NPVOffset              & 1 & Pile-up off-set substraction for primary vertices \\
%
JES  Pile-up  MuOffset               & 1 & Pile-up off-set substraction for number of expected interactions \\
% 
JES  Pile-up  Pt  term               & 1  & Pile-up jet area substraction technique \pt-term \\
%
JES  Pile-up  Rho  topology          & 1  & Pile-up jet area substraction technique event density uncertainty \\
%
\hline
Common sources in jet calibration          &  & \\
%
%
JES  Flavour  Comp                  & 1  & Quark/gluon jet composition difference between various MC event generators \\ 
%
JES  Flavour  Response              & 1  & Quark/gluon jet response difference between \pythia{} and \herwig \\ 
%
\hline
Jet energy resolution (JER) &  & \\
%
%
JER  DataMC  Difference             & 1 & Treats the case where data JER uncertainty is better than in MC \\
%
JER  NoiseInSitu                    & 1 & In situ determination of the noise fluctuation effect on JER \\
%
JER  NPi                            & 9 & Eigenvectors $i=0,8$ of the in situ techniques JER uncertainties  \\
%
\hline
Other sources &  &  \\
%
Unfolding  bias                     & 1 & Residual bias in the detector unfolding  \\     
%
JAR  jar                            & 1 & Jet angular resolution   \\           
%
mc  stat                            & 1 & Number of events in Monte Carlo simulation \\
%
jetcleaning  BCH                    & 1 & Jet cleaning for jets pointing to dead hadronic calorimeter modules  \\
%
\hline
\end{tabular}
}
\caption{
Summary table of the systematic uncertainty components 
for the jet energy scale (JES) and resolution (JER) together with
other uncertainties related to the jet measurement, the Monte Carlo event statistics and the detector unfolding.
Given is the name, the number of components ($N$) and a short description.
More information on the individual uncertainty in the JES and JER sources can be found in Ref.~\cite{ATLAS-CONF-2015-037}.
%
Except of the  Monte Carlo event statistics (mc  stat) uncertainty, all individual uncertainty
components are correlated across \pt and rapidity bins.
For the JES  EtaStati uncertainty the first (second) number refers to $R=0.4$ ($R=0.6$) jets.
%
}
\label{tab:JESuncertainty-sources}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

